Inferring Types for Parallel Programs

The Message Passing Interface (MPI) framework is widely used in implementing imperative pro- grams that exhibit a high degree of parallelism. The PARTYPES approach proposes a behavioural type discipline for MPI-like programs in which a type describes the communication protocol followed by the entire program. Well-typed programs are guaranteed to be exempt from deadlocks. In this paper we describe a type inference algorithm for a subset of the original system; the algorithm allows to statically extract a type for an MPI program from its source code.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{V.T. Vasconcelos and P. Haller (Eds.): Workshop on Programming Language\\ Approaches to Concurrency- and Communication-cEntric Software (PLACES'17)\\
EPTCS 246, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.246.6}{10.4204/EPTCS.246.6}}
\pdfoutput=1

